Language classification from bilingual word embedding graphs

We study the role of the second language in bilingual word embeddings in monolingual semantic evaluation tasks. We find strongly and weakly positive correlations between down-stream task performance and second language similarity to the target language. Additionally, we show how bilingual word embeddings can be employed for the task of semantic language classification and that joint semantic spaces vary in meaningful ways across second languages. Our results support the hypothesis that semantic language similarity is influenced by both structural similarity as well as geography/contact.

==> plots/german.tex <==
\begin{tikzpicture}[-,>=stealth',shorten >=1pt,auto,node distance=2.5cm,
  thick,main node/.style={circle,fill=blue!20,draw,minimum width=0.1cm, font=\sffamily\bfseries}]

  \begin{scope}
  \node[main node] (1) {cat};
  \node[main node] (2) [below left=0.3cm of 1] {dog};
  \node[main node] (3) [below right of=2] {man};
  \node[main node] (4) [below right=0.2cm of 1] {bear};
  \node[main node] (5) [below right=0.05cm of 3] {woman};
  
%  \node[main node] (5) [right= 3cm of 1] {5};
%  \node[main node] (6) [below left of=5] {6};
%  \node[main node] (7) [below right of=6] {7};

  \tikzset{Friend/.style   = {
                                 double          = green,
                                 double distance = 1pt}}
  \tikzset{Enemy/.style   = {
                                 double          = red,
                                 double distance = 1pt}}

%  \draw[line width=2mm, draw=green](1) to (2); 
%  \draw[line width=1mm, draw=green](1) to (3);
%  \draw[line width=0.5mm, draw=green](1) to (4);
%  \draw[line width=3mm, draw=green](2) to (3);
%  \draw[line width=2.5mm, draw=green](2) to (4);
%  \draw[line width=1mm, draw=green](3) to (4);

%  \draw[Friend](5) to (6);
%  \draw[Friend](5) to (7);
%  \draw[Friend](6) to (7);

%  \draw[Enemy](1) to (5);
%  \draw[Enemy](1) to (6);
  %\draw[Enemy](1) to (7);
%  \draw[Enemy](3) to (6);
%  \draw[Enemy](3) to (7);
%  \draw[Enemy](4) to (6);
  %\begin{pgfonlayer}{background}
  %  \filldraw [line width=4mm,join=round,black!10]
  %    (1.north  -| 2.west)  rectangle (3.south  -| 4.east)
  %    (5.north -| 6.west) rectangle (7.south -| 7.east);
  %\end{pgfonlayer}
\end{scope}
  \begin{scope}[xshift=5cm]
  \node[main node] (1) {cat};
  \node[main node] (2) [below left of=1] {dog};
  \node[main node] (3) [below right of=2] {man};
  \node[main node] (4) [below right of=1] {bear};

%  \node[main node] (5) [right= 3cm of 1] {5};
%  \node[main node] (6) [below left of=5] {6};
%  \node[main node] (7) [below right of=6] {7};

  \tikzset{Friend/.style   = {
                                 double          = red,
                                 double distance = 1pt}}
  \tikzset{Enemy/.style   = {
                                 double          = red,
                                 double distance = 1pt}}

  \draw[line width=2.2mm, draw=red](1) to (2); 
  \draw[line width=1.5mm, draw=red](1) to (3);
  \draw[line width=0.5mm, draw=red](1) to (4);
  \draw[line width=0.8mm, draw=red](2) to (3);
  \draw[line width=2.5mm, draw=red](2) to (4);
  \draw[line width=3.5mm, draw=red](3) to (4);

%  \draw[Friend](5) to (6);
%  \draw[Friend](5) to (7);
%  \draw[Friend](6) to (7);

%  \draw[Enemy](1) to (5);
%  \draw[Enemy](1) to (6);
  %\draw[Enemy](1) to (7);
%  \draw[Enemy](3) to (6);
%  \draw[Enemy](3) to (7);
%  \draw[Enemy](4) to (6);
  %\begin{pgfonlayer}{background}
  %  \filldraw [line width=4mm,join=round,black!10]
  %    (1.north  -| 2.west)  rectangle (3.south  -| 4.east)
  %    (5.north -| 6.west) rectangle (7.south -| 7.east);
  %\end{pgfonlayer}
\end{scope}
  \begin{scope}[xshift=10cm]
  \node[main node] (1) {cat};
  \node[main node] (2) [below left of=1] {dog};
  \node[main node] (3) [below right of=2] {man};
  \node[main node] (4) [below right of=1] {bear};

%  \node[main node] (5) [right= 3cm of 1] {5};
%  \node[main node] (6) [below left of=5] {6};
%  \node[main node] (7) [below right of=6] {7};

  \tikzset{Friend/.style   = {
                                 double          = blue,
                                 double distance = 1pt}}
  \tikzset{Enemy/.style   = {
                                 double          = red,
                                 double distance = 1pt}}

  \draw[line width=1.5mm, draw=blue](1) to (2); 
  \draw[line width=1.5mm, draw=blue](1) to (3);
  \draw[line width=3.1mm, draw=blue](1) to (4);
  \draw[line width=3.5mm, draw=blue](2) to (3);
  \draw[line width=2mm, draw=blue](2) to (4);
  \draw[line width=1.5mm, draw=blue](3) to (4);

%  \draw[Friend](5) to (6);
%  \draw[Friend](5) to (7);
%  \draw[Friend](6) to (7);

%  \draw[Enemy](1) to (5);
%  \draw[Enemy](1) to (6);
  %\draw[Enemy](1) to (7);
%  \draw[Enemy](3) to (6);
%  \draw[Enemy](3) to (7);
%  \draw[Enemy](4) to (6);
  %\begin{pgfonlayer}{background}
  %  \filldraw [line width=4mm,join=round,black!10]
  %    (1.north  -| 2.west)  rectangle (3.south  -| 4.east)
  %    (5.north -| 6.west) rectangle (7.south -| 7.east);
  %\end{pgfonlayer}
\end{scope}
\end{tikzpicture}

